Solving Mixed Integer Programs Using Neural Networks

Mixed Integer Programming (MIP) solvers rely on an array of sophisticated heuristics developed with decades of research to solve large-scale MIP instances encountered in practice. Machine learning offers to automatically construct better heuristics from data by exploiting shared structure among instances in the data. This paper applies learning to the two key sub-tasks of a MIP solver, generating a high-quality joint variable assignment, and bounding the gap in objective value between that assignment and an optimal one. Our approach constructs two corresponding neural network-based components, Neural Diving and Neural Branching, to use in a base MIP solver such as SCIP. Neural Diving learns a deep neural network to generate multiple partial assignments for its integer variables, and the resulting smaller MIPs for un-assigned variables are solved with SCIP to construct high quality joint assignments. Neural Branching learns a deep neural network to make variable selection decisions in branch-and-bound to bound the objective value gap with a small tree. This is done by imitating a new variant of Full Strong Branching we propose that scales to large instances using GPUs. We evaluate our approach on six diverse real-world datasets, including two Google production datasets and MIPLIB, by training separate neural networks on each. Most instances in all the datasets combined have $10^3-10^6$ variables and constraints after presolve, which is significantly larger than previous learning approaches. Comparing solvers with respect to primal-dual gap averaged over a held-out set of instances, the learning-augmented SCIP is 2x to 10x better on all datasets except one on which it is $10^5$x better, at large time limits. To the best of our knowledge, ours is the first learning approach to demonstrate such large improvements over SCIP on both large-scale real-world application datasets and MIPLIB.

==> author_contributions.tex <==
\section{Author Contributions}
\label{sec:author_contributions}


People who contributed: \\
- Nicolas contributed to: Data Generation for Neural Branching; Implementation of DAgger for Neural Branching; visualization and analysis code for Neural Branching; implementation of evaluation code for cut selection expert. \\
- Pengming contributed to: Design & implementation of Neural Diving data generation, training and evaluation setup and model architectures, handling general integers, approach to finding MIPLIB incumbents \\
- Pawel \\
- Brendan: Neural branching, GCN, RL, TPUs, ADMM-based solver \\
- Ingrid contributed to: Design & implementation of Neural Diving data generation, training and evaluation setup and model architectures,
- Vinod \\
- Ivan contributed to: Implemented the proof-of-concept version of the Neural Diving end-to-end pipeline, proposed the initial version of the GCN-based efficient neural network architecture, further design & implementation of Neural Diving data generation, training and evaluation setup and model architectures, approach to finding MIPLIB incumbents.  \\
- Ravi: Implemented a proof-of-concept design for speeding up inference of the Neural Branching's GraphNet model by batching states from multiple nodes together and performing batched inference on a GPU. \\
- Felix: implemented visualization for Neural Branching, evaluated MIP Solving with different branching experts with SCIP, brainstormed and investigated and added neural architecture improvements, automated and managed data generation for training Neural Branching on SCIP 7.0.1, implemented a proof-of-concept RL training setup \\
- Sergey Bartunov: participated in development of data generation, model architectures, training as evaluation for Neural Diving. \\
- Christian \\
- Yori \\
- James Keeling \\
- Thomas Keck: designed and implemented supervised learning training setup for Neural Branching \\
- Jonathan Goodwin: gave advice on making graphnet training more scalable \\
- Yujia Li: implemented and trained a few initial GNN architectures, and gave advice on graph neural network architecture in general \\
- Ira: contributed to the graph data analysis and interpretability of the Neural Diving trained models \\
\felix{Include people involved in the extravaganza and people involved in improving engineering infrastructure and earlier projects}

==> batch_lp.tex <==

\section{Batched Convex Optimization}

\subsection{Scaling Up Strong Branching with Batched Solving of LPs}
- ADMM-based approach to solving LPs in a Strong Branching decision by batching them.\\
- By using GPUs, it becomes possible to scale up Strong Branching to large MIPs.\\
- Explain formulation.\\
- Show results on individual MIPs and speedup over classical Strong Branching.\\
- Show the MIPLIB results\\
- Present imitation learning accuracy results, but not solve performance, on various datasets to demonstrate that the expert policy can be learned.\\
- Give more details in the appendix.\\

In many practical uses of convex optimization we want to solve several similar
problems in parallel. Examples include control of a population of agents,
hyper-parameter sweeps, and mixed integer programming. In this manuscript we
focus on the case of applying branch and bound to a mixed integer programming
problem where we use full strong branching to select branching variables.  To
apply full strong branching we must solve $2n$ linear programs (LPs) in
parallel at every node, where $n$ is the number of unfixed integer variables.
These LPs differ by only one entry in the constraints. We show that these
problems can be batched together and solved simultaneously. The batching
allows the use of modern hardware accelerators such as GPUs and TPUs
and yields huge speedups compared to sequentially solving the LPs.

\section{Introduction}
First-order methods have become popular for solving large-scale convex
optimization problems that are prohibitively large for second-order methods
\cite{ocpb:16}. This report describes applying these methods and exploiting 
structure in the problems they are applied to in order to do batch computations
on modern hardware accelerators to provide large speedups over solving the
problems serially.
\subsection{Mixed integer programming}
In mixed integer programming the goal is to find an integer assignment to a
vector of variables that minimizes an objective, subject to additional
linear constraints, that is
\[
\begin{array}{ll}
\mbox{minimize} & c^T x\\
\mbox{subject to} & b_l \leq Ax \leq b_u\\
  & x \in \mathbb{Z}^n.
\end{array}
\]
over variable $x$. MIPs have a myriad of applications, including scheduling,
routing, planning, portfolio optimization \etc. Solving MIPs is typically
performed by solving many linear programs as part of branch and bound (explained
later) or cut generation routines. Indeed at least 80\% of the time solving a
MIP is spent solving LPs. In this manuscript we exploit
the structure of the LPs that are solved when solving MIPs in order
to reduce the overall MIP solving time. First we cover the algorithm
we shall use to solve linear programs.
\subsection{Branch and Bound}

\subsection{The alternating direction method of multipliers}
Consider the following composite convex optimization problem
\[
\begin{array}{ll}
\mbox{minimize} & f(x) + g(z)\\
\mbox{subject to} & x = z
\end{array}
\]
over variables $x \in \reals^n$, $z \in \reals^n$ and where $f : \reals^n
\rightarrow \reals \cup \{ \infty \}$, $g : \reals^n
\rightarrow \reals \cup \{ \infty \}$ are closed, proper, convex functions.
The \emph{Alternating direction method of multipliers} (ADMM) applied to this
problem is the following procedure for any $\rho > 0$:
\[
\begin{array}{ll}
  x^{k+1} &= \argmin_x \Big(f(x) + (\rho/2) \|x - z^k - \lambda^k \|_2^2\Big)\\
  z^{k+1} &= \argmin_z \Big(g(z) + (\rho/2) \|x^{k+1} - z - \lambda^k\|_2^2\Big)\\
\lambda^{k+1} &= \lambda^k + x^{k+1} - z^{k+1}.
\end{array}
\]
Under benign conditions this procedure converges to primal-dual optimal points,
\ie,
\[
x^k, z^k, \lambda^k \rightarrow x^\star, z^\star, \lambda^\star
\]
for any $\rho > 0$.
\subsection{Linear programming}
A linear program (LP) is the following convex optimization problem
\[
\begin{array}{ll}
\mbox{minimize} & c^T x\\
\mbox{subject to} & b_l \leq Ax \leq b_u\\
& l \leq x \leq u
\end{array}
\]
over variable $x \in \reals^n$, with data matrix $A \in \reals^{m \times n}$,
$b_l, b_u \in \reals^m$, $l, u \in \reals^n$, $c \in \reals^n$. 
We can write this problem in a form more amenable to ADMM:
\[
\begin{array}{ll}
\mbox{minimize} & c^T x + \Ic_{Ax = y}(x, y) + \Ic_{[b_l, b_u]}(\tilde y)+ \Ic_{[l, u]}(\tilde x) \\
\mbox{subject to} & \begin{bmatrix}x \\ y\end{bmatrix} = \begin{bmatrix}\tilde x \\ \tilde y\end{bmatrix}
\end{array}
\]
where $\Ic_\Xc$ denotes the convex indicator function of set $\Xc$, \ie,
\[
  \Ic_\Xc(z) = \left\{
    \begin{array}{rl}
      0 & z \in \Xc \\
      \infty & {\rm otherwise.}
    \end{array}
    \right.
\]
When ADMM
is applied to this problem it yields the algorithm (though there are many
equivalent choices) over iterates $x, \tilde x \in \reals^n$, $y, \tilde y \in
\reals^m$, $\lambda \in \reals^{m+n}$:
\[
\begin{array}{ll}
(x^{k+1}, y^{k+1}) &=
\argmin_{Ax = y}
\left(
c^Tx +
\rho/2 \left\| \begin{bmatrix}x \\ y\end{bmatrix} - \begin{bmatrix}\tilde x^k \\
  \tilde y^k\end{bmatrix} - \begin{bmatrix}\lambda_x^k \\ \lambda_y^k\end{bmatrix} \right\|_2^2
\right)\\
\tilde x^{k+1} &= \Pi_{[l, u]}(x^{k+1} - \lambda_x^k)\\
\tilde y^{k+1} &= \Pi_{[b_l, b_u]}(y^{k+1} - \lambda_y^k)\\
  \begin{bmatrix}\lambda_x^{k+1} \\ \lambda_y^{k+1}\end{bmatrix} &=
    \begin{bmatrix}\lambda_x^k \\ \lambda_y^k\end{bmatrix}+ \begin{bmatrix}x^{k+1} \\ y^{k+1}\end{bmatrix} - \begin{bmatrix}\tilde x^{k+1}\\ \tilde y^{k+1}\end{bmatrix}
\end{array}
\]
Note that only first step is computationally challenging, which for some RHS $r
\in \reals^{m+n}$ can be performed using
\[
  (x^{k+1}, y^{k+1}) = \argmin_{Ax = y} \left(c^Tx + \rho/2 \left\| \begin{bmatrix}x \\
    y\end{bmatrix} - \begin{bmatrix}r_x^k \\ r_y^k \end{bmatrix} \right\|_2^2\right)
\]
\[
  \begin{bmatrix}x^{k+1} \\ y^{k+1} \end{bmatrix} =
\begin{bmatrix}
I & A^T \\ A & -I
\end{bmatrix}^{-1}
\begin{bmatrix}
r_x^k - c / \rho \\ 0
\end{bmatrix} +
\begin{bmatrix}
0 \\ r_y^k
\end{bmatrix}
\]
Note that the matrix is the same \emph{for all iterations}, this will be
    important when we discuss batching. There are two options
    for inverting the matrix:
\BIT
\item direct: (sparse) factorize once and reuse $M = LDL^T$
\item indirect: (sparse) conjugate gradients on PSD reduction $(I+ A^T A)$.
\EIT
\subsection{Full strong branching}
Now we come to the main application area of this manuscript. In full strong
branching the goal is to identify the branching variable by solving the one-step
lookahead problem for each variable. That is, simulating the branching decision
by solving the linear programming relaxation with each variable branched to the
nearest integer values, both rounded up and rounded down. In other words,  
for each $i \in \Cc$ we solve two LPs with new variable bounds:
\[
\begin{array}{lr}
\begin{array}{ll}
\mbox{minimize} & c^T x\\
\mbox{subject to} & b_l \leq Ax \leq b_u\\
& {\color{red} l^{(i)}} \leq x \leq u
\end{array}
\begin{array}{ll}
\mbox{minimize} & c^T x\\
\mbox{subject to} & b_l \leq Ax \leq b_u\\
& l \leq x \leq  {\color{red} u^{(i)}}
\end{array}
\end{array}
\]
We have highlighted in the red the difference between the base LP and the new
    ones.  Moreover, note that the $A$ matrix identical for all LPs. We shall
    exploit this fact to batch the computation of the most expensive step
    together.
 With this we only need to factorize matrix once for all $i \in \Cc$, then we
    can rely on matrix-matrix ops and exploit faster kernels for these
    operations on GPU.  This yields hardware benefits for both direct and
    indirect approaches. GPUs are designed to provide very fast dense mat-mat
    multiply routines. However, sparse matrix operations are less efficient
    uses of the stream parallelism and consequently are slower. If we batch
    sparse mat-vec into mat-mat, then the GPU can be kepy busy by using the 
    fact that the right hand side is typically dense.
\subsection{GPU speedups}
Here we present speedup results on a single GPU for the MIPLIB dataset.
First we consider a single MIP from the MIPLIB dataset, the
air05 MIP at root node, which has 6.1k vars, 43.4k nnz, $98\%$ sparse.
We show the solve time vs batch-size on GPU, normalized by time for 1 LP
in Figure~\ref{f-air05}.
We show that we can compute all 12.2k branch scores in $<20 \times$ cost of 1,
which is approximately a $600\times$ speedup.
\begin{figure}[h]
\centering
  \includegraphics[width=0.7\linewidth]{figures/num_lps_v_time.png}
\caption{Solve time vs number of LPs in a batch.}
  \label{f-air05}
\end{figure}
Next we show that this pattern holds true for the entire MIPLIB dataset.
In Figure~\ref{f-hist} we show the histogram of the speedup, which is defined
as the time taken to solve all LPs at the root node divided by the time taken
to solve a single one. Note that we remove the effect of transferring the data
to the GPU, compiling the TensorFlow graph etc, by subtracting the time taken
to run zero iterations (which is non-zero) from denominator and numerator.
This figure shows that the speedup is significant across the board,
averaging aproximately $800\times$, almost three orders of magnitude.
\begin{figure}[h]
\centering
  \includegraphics[width=0.7\linewidth]{figures/miplib_hist.png}
\caption{Histogram of speedup factors for all MIPs in MIPLIB at root.}
  \label{f-hist}
\end{figure}
\subsection{Accuracy}
Warm-starting from the solution at the previous node means not many iterations
required for reasonable accuracy, which is a typical property of ADMM.
In Figure~\ref{f-accuracy} we plot two quantities at the root node of the air05
MIP, at which we need to solve approximately $12k$ LPs. On the left hand side
we plot the correlation of the $12k$ \emph{true}
objective values with the objective values returned by ADMM after a fixed
number of iterations. As we can see it converges towards one as the number
of iterations increases, but even for few iterations it is quite high,
indicating that we have a reasonable signal on the `good' branch and bound
variables with relatively little computational effort. On the right we show the
scatterplot of the true objective values and the objective values returned by
ADMM after $50$ iterations, and we can see the high correlation visually.
\begin{figure}
  \includegraphics[width=0.5\textwidth]{figures/iter_v_corr.png}
   \hfill
  \includegraphics[width=0.5\textwidth]{figures/12k_corr_50_iters.png}
\caption{Correlation of ADMM objective and true objectives at root of air05 MIP.}
\label{f-accuracy}
\end{figure}
\subsection{Results}
Here we present results on speed when using our LP solver as the solver
in Full strong branching, compared against SCIPs fullstrong branching and
reliable pseudo-cost branching, on several datasets: Neural network
verification, BCOL, and a combined 2010 and 2017 MIPLIB. The results are
presented as cactus plots in Figure~\ref{f-results}. In these plots
being lower and to the right indicates better performance, and note that
the y-axis shows time to solve (up to the tolerance) and is in a log-scale.
As can be seen, our policy is almost uniformly faster (by a significant margin)
on NN verification and BCOL, and is competitive in the gold-standard benchmark
MIPLIB dataset.
\begin{figure}[h]
\centering
  \includegraphics[width=0.5\linewidth]{figures/miplib_cactus.png}
  \hfill
  \includegraphics[width=0.5\linewidth]{figures/nn_cactus.png}
  \hfill
  \includegraphics[width=0.5\linewidth]{figures/bcol_cactus.png}
\caption{Cactus plots for timing performance results across three datasets.}
\label{f-results}
\end{figure}


==> introduction_old.tex <==

\section{OLD Introduction (use introduction_new.tex)}
\label{sec:intro}

\begin{figure}[t]
    \includegraphics[trim={3cm 2.5cm 3cm 2.5cm}, clip, width=0.98\textwidth]{figures/intro_overview.pdf}
    \caption{\small{Overview of our approach. We construct two neural network-based components to be used in a MIP solver, \emph{Neural Diving} and \emph{Neural Branching}. Neural Diving uses a generative model which, given the MIP to be solved, generates partial assignments for its integer variables. The resulting ``sub-MIPs" for un-assigned variables are then solved in parallel to construct high-quality complete assignments for the original input MIP. The generative model is trained on pairs of MIPs and feasible assignments (not necessarily optimal) precomputed with an off-the-shelf solver. Neural Branching is a learned policy that conditions on a leaf node of the current search tree to pick the next integer variable to branch on. It guides the tree search to quickly produce a short proof for how far the solution produced by Neural Diving is from optimum. The policy is trained to imitate an expensive ``expert'' policy, Full Strong Branching, that is designed to produce small trees. Combining the two produces a \emph{Neural MIP solver} which is customized to the distribution of MIPs for the application of interest. Results show that such a solver outperforms the solver SCIP, even after tuning SCIP's parameters for each application and even when the parallel computation of Neural Diving is performed sequentially. %
    }}
    \label{fig:overview}
\end{figure}

Mixed integer programs (MIPs) are a class of NP-hard problems where the goal is to minimize a linear objective subject to linear constraints, with some or all of the variables constrained to be integer-valued \citep{wolsey1998integer, karp1972reducibility}. Despite the fact that solving a MIP may take time exponential in the problem size, they have enjoyed widespread adoption in a broad range of applications, such as bin packing, capacity planning, resource allocation, and many others \citep{taha2014integer, junger200950, sierksma2015linear}. Significant research and engineering effort has gone into developing practical solvers, such as SCIP \citep{gamrath2020scip}, CPLEX \citep{cplex2009v12}, Gurobi \citep{gurobi2020}, and Xpress \citep{xpress}. These solvers rely on handcrafted, general-purpose heuristics developed by the community over several decades, and the ability of a solver to provide good solutions quickly depends strongly on the performance of such heuristics.

In industrial usage a MIP is rarely solved in isolation. Instead, an application typically requires solving a large set of similar MIPs. Real-world examples of this include selecting power plants on an electric grid to meet demand \citep{oneill17}, assigning cargo to flights \citep{li2012aircargo}, verifying a neural network's predictions across a set of inputs \citep{cheng2017verification, tjeng2018evaluating}, etc. For a given application, some problem parameters may remain largely the same across instances (e.g., in an electric grid, the set of available power plants and grid topology may not change), while others (e.g., fuel costs, electricity demand, etc.) may vary.
Off-the-shelf MIP solvers cannot automatically exploit this shared structure across instances, so in challenging applications users typically resort to handcrafting new heuristics or risk sacrificing performance. This can often provide large performance improvements, though at the expense of significant human effort and expertise.


In this paper we demonstrate that machine learning can provide application-specific heuristics that significantly outperform general-purpose ones used in a MIP solver, specifically the state-of-the-art open-source solver SCIP 7.0.1 \citep{gamrath2020scip}. Moreover, learning makes it possible to \emph{automatically} construct them from data, eliminating the need for human experts to handcraft new ones.
We evaluate our approach on five real-world application datasets, including two applications from Google's production systems, as well as the MIPLIB benchmark \citep{gleixner2019miplib}. Many of the MIPs in these datasets have a number of variables and constraints in the range of $10^4$--$10^6$ after presolve. To the best of our knowledge this is the first work to show that learning can improve solver wall-clock performance on such large-scale instances from real-world applications. \todoct{See my abstract comment; leaving this here as a reminder if we change this type of sentence.} 

Given a MIP with a nonempty set of joint variable assignments satisfying all the constraints, a solver needs to output such an assignment, and a proof bounding the gap in objective value between that assignment and an optimal one. We use \emph{Neural Diving} to find high quality joint variable assignments, and \emph{Neural Branching} to guide a tree search procedure to generate the proof. %

\paragraph{\textbf{Neural Diving:}} We train a deep neural network to produce partial assignments of the integer variables of the input MIP to be solved. The remaining unassigned variables define a smaller `sub-MIP', which is solved using an off-the-shelf MIP solver to complete the assignment. The model is trained to give higher probability to feasible complete assignments that have better objective values, using training examples collected offline with an off-the-shelf solver. It learns on all available feasible assignments instead of only the optimal ones, and does not necessarily require optimal assignments, which can be expensive to collect. At test time, it is used to sample multiple partial assignments and the subsequent sub-MIPs can be solved in parallel. 

This approach is a form of \emph{primal heuristic} \citep{berthold2006thesis}, which is a class of search heuristics used by MIP solvers to find feasible assignments. They have been identified as a key component that makes MIP solvers effective \citep{berthold2013primal}. Several works have focused on learning primal heuristics \citep{khalil2017primal, ding19accelerate, hendel2018adaptive, hottung2019neurallns, song2020generallns, addanki2020nlns}. Unlike these works, we pose the problem of predicting variable assignments as a generative modelling problem. This naturally lends itself to sampling multiple assignments and exploiting an existing solver to solve the sub-MIPs.

\paragraph{\textbf{Neural Branching:}} State-of-the-art MIP solvers use a form of tree search called \emph{branch-and-bound} \citep{Land1960BranchAndBound} (see \S \ref{sec:background}) over assignments of integer variables. The choice of the variable to branch on at a given node is a key factor in determining search efficiency \citep{achterberg2005branching, Glankwamdee2011LookaheadBF, schubert2017thesis, yang2019multivariablebranching}. We train a deep neural network policy to imitate choices made by an expert policy. The imitation target is a well-known policy called Full Strong Branching (FSB), which has been empirically shown to produce small search trees \citep{achterberg2005branching}, though it is often too computationally expensive for practical use. Once trained, the neural network is able to approximate the expensive policy at test time at a fraction of the computational cost.

Several works have looked at learning a branching policy \citep{He2014LearningToSearch, Khalil2016LearningToBranch, Alvarez2017MLApproxStrongBranching, balcan18learningtobranch, gasse2019exact, Yang2020LearningGS, zarpellon2020parameterizing, gupta2020hybrid}. Many of these focus specifically on learning to imitate FSB as we do \citep{Khalil2016LearningToBranch, Alvarez2017MLApproxStrongBranching, gasse2019exact}. Our approach differs from prior work in two important ways. First, we develop an approximation to FSB using the alternating directions method of multipliers (ADMM) \citep{boyd2011distributed} that scales to large-scale MIPs by performing the required computation in a batch manner on GPU. Second, unlike classical solvers which use branch-and-bound for the dual purposes of finding high-quality assignments as well as proving the optimality gap, we rely on the branching policy only for proving the gap \todoct{This sounds vague to me. What does it mean to use the branching policy only for gap?}, and use the Neural Diving to find high-quality assignments.  

We use SCIP's branch-and-bound implementation to apply Neural Branching to a MIP, as done by \cite{gasse2019exact}, and also use it as the sub-MIP solver for Neural Diving. There are two reasons for choosing SCIP: 1) Its API gives extensive access to its internal state for integrating learned models, and 2) its permissive licensing allows us to perform a large-scale evaluation by running solver instances in parallel.
The fact that we have implemented our techniques within SCIP makes SCIP the fairest baseline to compare against.
We have not yet compared our approaches to any commercial solvers, except for a partial evaluation of Neural Diving against Gurobi in section \ref{sec:supermip}. It shows that Neural Diving with Gurobi as the sub-MIP solver outperforms Gurobi. %

\subsection{Contributions}
\label{subsec:contributions}
\begin{enumerate}
    \item We propose Neural Diving (section \ref{sec:supermip}), a new learning-based approach to generating high-quality complete variable assignments
    for a MIP. On the application-specific datasets, Neural Diving achieves an average primal gap of 1\% on a held out set of instances 3-10$\times$ faster than SCIP with its emphasis parameters tuned to each dataset. (On one dataset SCIP does not reach 1\% average primal gap within the time limit, while Neural Diving does.) A comparison to Gurobi on two datasets also shows 3$\times$ and 3.6$\times$ less time to reach 1\% average primal gap using our approach. We have applied a modified version of the approach to a subset of open instances in MIPLIB to find three new best known solutions, beating commercial solvers.
    \item We propose a new scalable expert policy based on ADMM (section \ref{sec:deep_Branching}) to use as the imitation target for learning a branching policy which exploits GPUs to make imitation data generation from large MIPs computationally tractable. On two of the datasets in our benchmark for which FSB is slow due to large instances (e.g., with $> 10^5$ variables) or high iteration times, the new expert generates 1.4$\times$ and 12$\times$ more training data in the same running time. This allows scaling up the imitation learning approach to large-scale, challenging datasets.
    \item Using the data generated by our expert we train a deep graph neural network that makes decisions
    in a branch-and-bound tree. This Neural Branching policy (section \ref{sec:deep_Branching}) has comparable or better performance to the state-of-the-art branching heuristic in SCIP across all datasets we tested.
    \item We combine Neural Diving and Neural Branching (section \ref{sec:joint_eval}) to attain significantly better running time performance than SCIP across \emph{all} our test datasets, as measured by the average gap between primal and dual bounds on held out instances. At large time limits, the average gap is about $2\times$ to $10\times$ better than that of SCIP, with one dataset showing a $10^6\times$ improvement. Surprisingly, a $2\times$ improvement is seen even on MIPLIB 2017's Benchmark Set which, unlike the other datasets we use, consists of mostly unrelated, heterogeneous instances from many distinct problem families. %
    \item We plan to open source two of the datasets, for the applications of Neural Network Verification and Electric Grid Optimization, which we hope will help further research on new learning techniques for MIPs.
\end{enumerate}





















==> limitations.tex <==

\section{Limitations}
\label{sec:limitations}
Explain limitations of each part of the paper together at this point.

Limitations of Neural Branching:
\begin{enumerate}
    \item Behavioural cloning can be susceptible to policy errors at test time causing the test state distribution to become significantly different from the training one, in turn affecting the policy's performance. More sophisticated imitation learning techniques that use rollouts from the policy during training can address this.
    \item The expert policy is not provably optimal and our approach will not discover a better one even if it exists. The policy trained with imitation learning can be fine-tuned further using reinforcement learning to address this.
    \item Better architectures and algorithms that improve the generalization of the policy are needed to handle broad instance distributions arising from a diverse set of applications.
\end{enumerate}

Limitations of Neural Diving:
\begin{enumerate}
\item \textbf{Homogeneous labelled data:} Since our approach uses supervised learning of a variable prediction model, it relies on the existence of a labelled dataset of homogeneous MIP instances (i.e. with optimal or feasible solutions already known). In Google production use cases, it is common to repeatedly solve MIP instances of a similar type (e.g. index placement). The instances need not have the same number of variables and constraints (the predictor is independent of this due to the graph net)

\item \textbf{No proof of optimality:} This approach is designed to quickly find acceptable solutions to the MIP, but does not prove optimality of solutions. This method could be used in combination with a branch-and-bound solver which is optimised to find tight dual bounds.
\end{enumerate}

==> outline.tex <==


\paragraph{Learned primal heuristics.}


\paragraph{Learned branching rule.}
In this work we explore how to use learning to speed up a MIP solver. Specifically, we look at learning a branching policy to be used in a tree search algorithm for solving a MIP instance. The quality of the branching policy affects the running time of the solver significantly as it determines the number of search steps needed to solve a problem instance. We use imitation learning to train a neural network to imitate a step-efficient expert policy. The expert policy we use is computationally too expensive to be practically useful as a branching policy itself. But it can still be used to generate imitation training data for distilling it into a neural network. Learning on MIP instances sampled from a highly structured distribution can exploit the similarities among them to construct a computationally efficient approximation to the expert policy.

The branch and bound algorithm can be viewed as a sequential decision process in which the \emph{observation} is the current node where a branching decision is to be made, the \emph{action} is to select a variable to branch on, and the \emph{environment} updates the search tree by adding two new nodes based on the branching action and then selects the next node to branch on, which is output as the next observation (figure~\ref{fig:bab_mdp}). Our approach is to learn a branching policy to imitate an expert policy via behavioural cloning. Its key elements are described below.

\paragraph{Learned cut selection.}




\section{Learning a Variable Selection Policy}
- Learn a neural network to select variables at a given node during branch and bound.\\

\subsection{Imitation Learning}
- Main variants: 1) Behavioral Cloning (BC), 2) BC + random moves, 3) DAGGER.\\
- Distill an expensive-but-step-efficient variable selection policy into a neural network which can run significantly faster.\\
- Behavioral Cloning is not robust to shifts away from the expert's state distribution. This is particularly problematic in the case of branching as mistakes near the root can cause the state to be far away from the expert's distribution. Mixing random moves with expert moves and DAGGER address this limitation.\\ 

\subsection{Imitation learning accuracy}
The graph neural network is able to predict the Full Strong Branching decisions with accuracy much higher than chance. We use top-10 accuracy as the metric, which measures the percentage of branch and bound tree nodes on which the network ranks the Full Strong Branching policy's decision as one of the top 10 most probable decisions. See table~\ref{tab:validation_top10_accuracy}. That it is possible to learn at all on such large scale graphs is reassuring, given that such an experiment has not yet been attempted in the domain of learning on mixed integer programs.  Note that the training set results are only a few percentage points better than the validation set results, so currently the graph neural network is underfitting on all four datasets. We hope to improve the results further using larger models. Although the accuracies are far below 100\%, it is still possible that a poor approximation of Full Strong Branching can still improve the MIP solver performance over using the default policy used in SCIP, especially if the graph neural network is able to provide better branching decisions near the root of the branch and bound tree which has a stronger influence on the solver performance.
\begin{table}
    \centering
    \begin{tabular}{c | c | c}
    \toprule
        Dataset & Top-1 & Top-10\\
        & validation & validation \\
        & accuracy & accuracy \\
        \midrule
        MIPLIB & 33.7\% & 52.5\% \\
        OR & 43.8\% & 69.9\% \\
        NN Verification & 32.6\% & 67.2\% \\
        Blokus Packer & 6.8\% & 11.2\%\\
    \bottomrule
    \end{tabular}
    \caption{\% Top-10 accuracy for predicting Full Strong Branching decisions on branch and bound tree nodes from MIP instances in the validation set of each dataset.}
    \label{tab:validation_top10_accuracy}
\end{table}


\begin{figure}[t]
    \begin{tabular}{cc}
        \includegraphics[width=0.5\textwidth]{figures/cactus_plots.png}\\
    \end{tabular}
    \vspace{-0.2in}
    \caption{
        {\small Comparison of the wall clock solving time for \textcolor{red}{Full Strong Branching}, \textcolor{green}{Reliable Pseudocosts Branching}, which is SCIP's default, and a \textcolor{blue}{learned policy} on the MIPLIB, OR, Blokus Packer, and NN Verification test sets. The number in paranthesis in subfigure titles is the number of MIP instances being solved. A policy that solves more MIP instances faster will have a curve that is shifted more to the bottom right than other policies. The graph neural network policy is able to match or slightly improve on SCIP's default policy on the Blokus Packer and NN Verification test sets, while it is significantly worse on MIPLIB and OR test sets.}
    }
    \label{fig:cactus_plots}
\end{figure}




\subsection{Results}
- Present learning curves for the conditional generative model on all six datasets.\\
- Present solving time results on all six datasets, comparing to only SCIP (no Gurobi) and a simple baseline that replaces the learned model's predictions with random choices to demonstrate the effect of learning.\\

\section{Learning to Select Cuts}
- We focus on selecting cuts at the root node.\\
- Learn to imitate a Strong Cutting policy.\\
- Absolute scoring versus relative scoring.\\

\subsection{Results}
- Show dual bound improvements on the test set for all six datasets, both at the root node and after branch and bound.\\
- Compare to SCIP adding the same number of cuts at the root node.\\
- Show the effect of varying the number of cuts added at the root.\\

\section{Putting the Pieces Together}
- We use branching and cut selection in order to improve the lower bound, and solution prediction as a primal heuristic that runs in parallel to branch and bound.\\






==> raw_results_par10.tex <==
\begin{verbatim}
CORLAT
Full Strong,16.218206043258
Neural Branching,132.93809930691359
Neural Branching + Neural Diving (Sequential),6.013353603548653
Tuned SCIP,12.084287437641082
Tuned SCIP + Neural Diving (Sequential),5.293666811143371

NN Verification
Full Strong,2375.7642450845105
Neural Branching,21.72229438535693
Neural Branching + Neural Diving (Sequential),10.2049813085634
Tuned SCIP,7812.809258695501
Tuned SCIP + Neural Diving (Sequential),2813.326468782675

MIPLIB
Full Strong,59332.451579076274
Neural Branching,55640.03416875147
Neural Branching + Neural Diving (Sequential),43989.3343288185
Tuned SCIP,45685.6725043093
Tuned SCIP + Neural Diving (Sequential),32572.184905693157

Packing
Full Strong,80899.38978460226
Neural Branching,80856.83418889214
Neural Branching + Neural Diving (Sequential),56738.13936401463
Tuned SCIP,80462.69195464902
Tuned SCIP + Neural Diving (Sequential),58758.44814134814

Grid
Full Strong,11223.372160397248
Neural Branching,2311.019490384434
Neural Branching + Neural Diving (Sequential),2450.803163231129
Tuned SCIP,3697.807352350929
Tuned SCIP + Neural Diving (Sequential),3279.348671184918

Planning
Full Strong,57157.97177480832
Neural Branching,56459.13926735947
Neural Branching + Neural Diving (Sequential),49524.11202405421
Tuned SCIP,52354.823820345206
Tuned SCIP + Neural Diving (Sequential),49642.66677585531
\end{verbatim}

==> rep_and_arch_OLD.tex <==


\section{Input Representation and Network Architecture}
We describe how a MIP is represented as an input to a neural network, and the architecture we use to learn models for both Neural Diving and Neural Branching.

\subsection{MIP Representation}
The MIP in equation~\ref{eqn:mip1} can be represented as a bipartite graph, where one set of $n$ nodes in the graph correspond to the $n$ variables being optimized, and the other set of $m$ nodes in the graph correspond to the $m$ constraints. The edges between the nodes indicate which variables belong to which constraints. This MIP representation is used for learning by \cite{gasse2019exact, ding2019accelerating}, and an analogous representation for Boolean Satisfiability is used earlier by \cite{selsam2019NeuroSAT}.  

\TODO{important: what is a `feature'? the word is used many times here but never defined.} The values in the constraint matrix $A$ are represented as edge features \felix{was our constraint matrix row- and column- normalized? where should we mention that?}, while the values in the objective vector $c$ are represented as features of the corresponding variable nodes, and the values in the constraint vector $b$ are represented as features of the corresponding constraint nodes \felix{where are we explaining the exact set of features we use?}. Additional information, such as the values assigned to variables and the values of the variables in the linear program solution, can be represented as node features. The bipartite graph representation of the MIP forms the input to the neural network branching policy.

\subsubsection{Feature extraction and graph representation of MIPs}
\label{sec:NNS_features}

\TODO{THIS SECTION NEEDS TO BE MERGED WITH THE REST OF THE TEXT.}

\begin{figure*}
    \centering
    \includegraphics[trim={1cm 4cm 1cm 1cm},clip,width=\textwidth]{figures/MIP_GNN.pdf}
    \caption{An integer program can be represented as a bipartite graph such that one set of nodes represent variables, the other set constraints, and edges correspond to the non-zeros of the constraint matrix. $\{A, b, c\}$ can be encoded as features of the graph's nodes and edges. A \emph{graph neural network} takes the graph and its node and edge features as input and computes a fixed dimensional continuous vector for each node. These vectors can then be used to make node-specific predictions.}
    \label{fig:mip_gnn}
\end{figure*}


We represent MIP instances as bipartite graphs, following the Constraint-Variable Incidence Graph (CVIG) model (\cite{ansotegui2012}): each variable and each constraint is represented as a node in the graph, and edge connections are defined using the constraint matrix $A$ as the adjacency matrix for the graph.
Node features contain the type of the variable (general integer, binary or continuous), its objective coefficient, and LP relaxation features (solution value in LP solution, fractionality in LP solution, etc.). 
Constraint features contain the right-hand side of the constraint, its similarity to the objective vector, and LP relaxation features. For the full list of features, we refer to \cite{gasse2019exact}. 
All these features are computed using SCIP~\cite{gleixner2018scip}. 

Once the basic features are extracted, we pass them to a $T$-layer graph neural network described next.
We treat embeddings \TODO{embeddings? again this needs to be defined} for variable nodes after $T$ rounds of message passing as the input features for all further computations in our generative models and denote them as $\mathbf{v}_d$ \TODO{what is $\mathbf{v}_d$? what space is it in \etc. Look at how we define the variables in the formulation of the problem, eg, `over variable $x \in \reals^n$, where $A \in \mathbb{R}^{m \times n}$, $b \in \mathbb{R}^m$, $c \in \R^n$ , $l \in \reals^n \cup \{-\infty\}^n$, and $u \in \reals^n \cup \{\infty\}^n$ are given data' - we need to be that rigorous for every mathematical quantity}.



\subsection{Neural Network Architecture}
\label{subsec:architecture}

A key limitation when considering network architecture is the memory footprint of the model during training on accelerator devices (\eg, GPU). A single accelerator device has finite memory and using several accelerators for training on a single sample can incur significant communication costs. Realistic MIP sizes require need a model that can tackle \TODO{this number is lower than the one we give in the intro} up to a hundred thousand nodes (number of variables plus constraints) and millions of edges (non-zero constraint coefficients). A general graph neural network's architecture \citep{battaglia2018relational} memory usage is $O(|\text{nodes}| + |\text{edges}|)$ which would be prohibitive for our use case. To sidestep this limitation we restricted ourselves to considering variants of GCN \TODO{what does GCN stand for?} \citep{kipf2016semi} which uses simple sparse-matrix multiplication instead of expensive edge blocks \TODO{edge blocks? never defined. and saying 'sparse multiplication' suggests other variants use 'dense multiplication' but what we actually mean is scalar vs matrix right?}\felix{Indeed, our node updates involve $tf.sparse.sparse_dense_matmul(adj\_mat, node\_embeddings)$}\felix{edge blocks are from DM's GraphNetworks terminology} and requires $O(|\text{nodes}|)$ in additional memory consumption (we still need to store the input edge features but do not store in accelerator-memory anything related to edges (of size $O(|\text{edges}|)$ beyond that \TODO{this is unclear, we don't store \emph{anything}?}\felix{Is this clearer?}). This fits our use-case especially well because our edges have only single scalar feature - constraint coefficient - which we used as coefficients in the adjacency matrix \TODO{very messy}. \\

Our graph network consists of several stacked layers, each of which consists of:
\begin{enumerate}
  \item 2-layered MLP with ReLU activations \citep{relu2010};
  \item Sparse multiplication by adjacency matrix $A$ \TODO{important: is this different to the $A$ matrix we're using in the MIP definition? If so it needs a real definition and another symbol}\felix{this is the adjacency matrix after presolving and possibly row/column normalized and specifically related to the current branching-node} where non-zero values are constraint coefficients (thus, variable nodes are connected only to constraint nodes and vice versa, the diagonal is zero);
  \item Dropout \citep{dropout2014};
  \item Skip connection \citep{skip_connections2016}: either through summation, concatenation, or a GRU cell that treats input to the layer as previous state and updated node features as a current input; 
  \item Layer norm \citep{layer_normalization2016} applied to the input or to the output of the layer.
\end{enumerate}
The difference between our approach and the original GCN is that we use more than a single layer in MLP and we allow the model to be more flexible with how to propagate node features via skip connections.
Thus an example of a single layer of node updates with layer norms applied to the output and GRU skip connections would be:
\begin{equation}
\begin{array}{rlcrl}
    \hv^{0}&=W_{\text{proj}}\xv, \\
    \hv_\msg^{(t+1)} &= \Dropout(A \; \MLP(\hv^{(t)})), \\
    \hv^{(t+1)}&=\LayerNorm(\GRU(\hv_\msg^{(t+1)}, \; \hv^{(t)})).
\end{array}
\end{equation}
For every task and dataset we do a grid search over architecture hyperparameters: number of layers, width of MLP layers, type of skip connection (summation, concatenation, or a GRU), location of the layer norm (before or after the layer). The best hyperparameters per task per dataset are reported in (\TODO{fill this}).

\TODO{can we delete these other tiny subsections? if not they need a lot of work}\felix{These are mainly a report for us, and a reproducibility aid, but they can be deleted safely, but the other architectures we tried section maybe should be even before the architecture description if reviewers will complain about why this particular thing, }

\subsubsection{Intuition}
As the elements of the adjacency matrix  $A$ are normalized, doing the multiplication by $A$ "aggregates" node embeddings with their neighbours according to the importance/contribution of the connections.

\subsubsection{General hyperparameter findings}

When the number of graphnet layers was between 0 and 16 increasing it by 2 (as the input graphs are bipartite) led to an increase in post-training test accuracy and decrease in test loss, going over 16 didn't lead to clear benefits.

Post-layernorm worked better than pre-layernorm which worked better than no layernorm normalization.

If memory allowed, having skip connections from earlier layers to later layers, via concatenation, worked best. 

\subsubsection{Other architectures we tried}

We tried several examples of general graph neural networks that had edge block computation, the one presented here based on sparse matrix multiplication worked better accuracy-wise and training-latency-wise.

We tried randomly initializing the graphnet and leaving it untrained, and only training the final mapping of representation to logit, which was faster to train but slightly worse in post-training test accuracy. Said trade-off may be desirable in some cases.


\subsubsection{Ablations we have not done}

We haven't done experiments trying to ascertain the minimal set of input features needed for the learning architecture to do well, for example we didn't try replacing the edge feature with a binary indicator and then measured the change in approximation quality.

We didn't try decoupling the feature transformation via MLP and the message passing via adjacency matrix multiplication, it is possible that the graph-structure information needed doesn't require the graph-node features, we haven't tested this hypothesis but if true it would allow having simpler learning models and possibly using symbolic methods on the same graph-structure information.

==> rl.tex <==

\section{Reinforcement Learning}

\subsection{MDP Formulation}
We formulate the problem of optimizing the dual bound of the MIP as a Markov Decision Process.\\
State = node of the branch and bound tree at which to select a variable to branch on.\\
Reward = dual bound at t - dual bound at t-1.\\
Action = select a variable at the current node.\\
Next state is given by the environment, which expands the tree by branching on the selected variable at the current node and then selects the next node to branch at.\\

==> supercuts.tex <==



\subsection{An expert for cut selection at the root of the branch-and-bound tree}
\label{subsec:supercuts}

An important component of MIP solvers are cutting planes (or cuts), whose role is to strengthen the LPs solved throughout the branch-and-bound tree. These cuts generally lead to smaller trees and help prove optimality faster, but they also increase the computational cost of the LPs. MIP solvers typically generate a large number of cuts and then use heuristics to identify the most useful ones to keep.
This latter process is called ``cut selection'' and its main purpose is to keep the size of the LPs in check. Cut selection
can also be helpful for numerical stability.

In this section, we report on an attempt to design an effective ``expert'' policy for selecting cuts
at the root node of the branch-and-bound tree. If we had such an expert, we could train a machine learning model
to imitate it, motivated by a similar line of reasoning as for the Neural Branching (see Section \ref{sec:deep_Branching}).
The expert is free to consume a large amount of resources in order to construct a good policy (just like Full Strong Branching does), because that step
is only done once in order to generate training data. The trained ML model will be used at test time or in 
practical applications, where resources are constrained, and the goal is to replicate the expert's performance at
a lower cost.

We emphasize that we did not generate any cuts, but only tried to design an expert to score cuts
generated by SCIP's cut algorithms in order to identify the most effective ones. The results we obtained show that
there is potential in this approach, but they were not conclusive enough yet to justify generating data and training
models. Therefore, we only report on experiments to assess the proposed expert's performance.

\subsubsection{A MIP Formulation for Cut Selection}

We now describe our attempt to design a cut selection algorithm that improves on the routines
used within SCIP at a higher computational cost. We set the goal of the expert to maximize the dual bound at the root, assuming a minimization problem. This expert does not take into account other considerations such as numerical stability, cut sparsity, diversity or orthogonality between cuts, and their performance throughout the branch-and-bound tree. Nevertheless, tightening the dual bound is an important effect of cuts, and these other considerations could be examined in further extensions to this expert.

Consider a mixed-integer linear program in the form of~\eqref{eqn:mip1} and suppose that we have a large pool of $\hat{m}$ cuts $\hat{A}x \leq \hat{b}$. We would like to select $k$ cuts from this pool such that the optimal value after adding these cuts to the LP is as tight as possible.

We can state this as the following problem. Define $z \in \{0,1\}^{\hat{m}}$ to be a binary variable that indicates which $k$ cuts are selected. Let $S_k = \{z \in \{0,1\}^{\hat{m}}\ |\ \sum_{i=1}^{\hat{m}} z_i = k\}$. Then the problem can be formulated as:
\begin{align*}
    \max_{z \in S_k} \min_x \{c^\top x\ |\ Ax \leq b, \hat{A}x \leq \hat{b} + M(1-z)\}
\end{align*}
where $M$ is a sufficiently large value. Note that setting $z_i$ to 0 relaxes the cut $i$, whereas setting it to 1 enforces it. If the problem is unbounded, there may not exist a large $M$ value that makes a given cut completely redundant, but in practice we can relax it enough so that it becomes ineffective.

To solve this problem as a single MIP, consider the dual view. From duality theory, given an optimal primal and dual pair of LP solutions, if a dual value is zero, then relaxing the corresponding constraint of the primal problem has no effect on the optimal value. If it is nonzero, then the corresponding inequality must be tight. Therefore, we consider the dual problem and enforce that only $k$ cuts can have nonzero dual values, which enables us to formulate this problem as a MIP:
\begin{align*}
    \max_{z \in S_k, y, \gamma} \{b^\top y + \hat{b}^\top \gamma\ |\ A^\top y + \hat{A}^\top \gamma = c,\ y \leq 0,\ \gamma \leq 0,\ \gamma \geq -Mz\}.
\end{align*}






\subsubsection{Evaluation Methodology}

There are two plausible ways in which the expert could
be harnessed in order to improve on SCIP's default cut selection. The first way is trying to obtain better dual
bounds with the same number of cuts, the goal being to obtain faster solving times by closing the primal-dual
gap in fewer steps. A second way of thinking about it is to obtain an approximately equal dual bound, but with fewer cuts. This might
lead to a branch-and-bound tree with more nodes, however the LPs considered throughout could be smaller, 
resulting in an improved solve time.

We performed experiments to test both approaches, focusing on letting the expert choose cuts at the root node only.
For the first way, we did not obtain conclusive evidence that the expert cuts help. A major disadvantage of the method is
that it is difficult to precisely control the number of cuts SCIP uses, as SCIP applies cuts in 
multiple rounds, and cuts selected in early rounds affect the generation and selection of later cuts.

The second method is easier to reason about, and does not involve modifying SCIP's default cut selection
when obtaining baseline results against which to compare the performance of the expert. In detail, the ``evaluate at root'' 
approach we pursued works as follows: For each MIP in our evaluation set and a specified 
number of cuts $n_c$, we run SCIP with a node limit of $1$, and used our expert to collect the best $n_c$ cuts from among all the
cuts in the cut pool at the end of processing the root node. All other SCIP settings are default and the cut selection MIP has a time limit of 6 hours. In a separate instantiation of the same MIP, those
$n_c$ cuts, and no other, are then applied at the root node via a custom separator. After the root node, SCIP may generate more cuts and manipulate the cuts from the cut pool and LP, as usual.


Carrying out this procedure for the range of values for $n_c \in \{50, 100, 200, 500\}$ and comparing the dual bounds achieved by SCIP with the 
ones obtained from the expert cuts alone, we derived, for each MIP, the smallest value for $n_c$ for which the 
expert dual bound was at least as good as SCIP's dual bound for at least one random seed. In a learning setting, a machine learning model may attempt to learn this parameter. For this particular set of experiments, the dual bound was matched with $n_c$ at most 500. All instances were run with 5 random seeds as discussed in Section~\ref{sec:evaluation}.

Armed with this information, we then ran the full evaluation process, as explained in Section \ref{sec:evaluation}
, with the following modification to take advantage of the expert cuts: For each MIP, we applied the
best $n_c^*$ expert cuts at the root, and no others, where $n_c^*$ was the smallest value for
$n_c$ determined earlier. We did not modify the cut generation or selection after the root node in any way.

\subsection{Results}


\begin{figure}[H]
 \begin{subfigure}[t]{.48\linewidth}
    \centering
        \includegraphics[width=.9\linewidth]{figures/supercuts/supercuts_avg_dual_gap_by_time_logy_no_root_time_hline_old.pdf}
    \caption{Average dual gap as a function of calibrated time on neural network verification instances.}\label{fig:supercuts_a}
  \end{subfigure}
  \begin{subfigure}[t]{.48\linewidth}
    \centering
        \includegraphics[width=.9\linewidth]{figures/supercuts/supercuts_surv_no_root_time.pdf}
    \caption{Survival plot with respect to calibrated running time. This plot only considers time after the root node.}\label{fig:supercuts_b}
  \end{subfigure}
  \caption{}\label{fig:supercuts}
\end{figure}
  

\begin{figure}[H]  
    \centering
        \includegraphics[width=.5\linewidth]{figures/supercuts/supercuts_cut_diff_hist.pdf}        
    \caption{Number of instances as a function of the difference between the number of selected cuts at the root and the number of cuts in the baseline.}\label{fig:supercuts_hist}
\end{figure}


In this section we present the results obtained using the methodology just
described. In all the results discussed in this section, the underlying dataset used was
NN Verification. Specifically, we used the MIPs from the NN Verification test set, as explained in
Section \ref{sec:datasets}.


Our main conclusion is that it is possible to obtain faster solving times overall by only applying
the expert cuts at the root node. Our hypothesis is that less time
is spent on solving LPs during the branch-and-bound algorithm, as the number of expert cuts we apply
at the root is typically lower than the number of cuts SCIP would have applied.

This is shown in the Figure \ref{fig:supercuts_hist}, which shows the distribution of the 
difference in the number of cuts applied at the root (i.e. number of expert cuts minus number of
default SCIP cuts) over the set of MIPs. Figure \ref{fig:supercuts_a} shows average dual gap curves, as defined in Section
\ref{sec:evaluation}, and we can see that for easier problems, with a solving time up to about $10^2$ seconds, using the root
cuts chosen by the expert produces a tighter dual gap. \todoct{Figure out if the improved gap already occurs at the root node. Do we have plots of root bound vs number of cuts?} Then for a window of time the baseline (without the expert
cuts) produces a slightly tighter dual gap, before the average drops below the $0.05$ target gap below which SCIP
terminates for a given MIP. The benefit of using the expert cuts is seen more readily in Figure \ref{fig:supercuts_b},
which shows the corresponding survival plots. 

Note that when we ran the full evaluation procedure using the expert cuts, we did not include the time required
to generate and select the expert cuts in the solving time. The justification is that eventually we plan
to replace the expert with a trained neural network, so rather than assessing the time performance of the expert
itself, we are interested only in the time performance of the branching process with the expert's cut choices.
Later on it will of course be crucial to include the time taken by the model to select the cuts, so as to obtain
a fair comparison. However, not including the time taken by the expert confers an unfair advantage; to
rectify this, we processed the data by subtracting the time taken to process the root node from both the expert
and the baseline run. 

We close this section by mentioning two related pieces of work. In \cite{tang2019LearningToCut}, the authors
train a reinforcement learning system to select Gomory cuts. The main differences to our work are that their algorithm
is not evaluated in the context of branch-and-bound, but either alone, by iteratively choosing cuts to add until
a given IP is solved, or in the context of branch-and-cut. The former approach especially
is only practical for very small problems,
which is another difference to our approach (the MIPs from the NN Verification set are considerably larger). Finally,
the authors compare their RL system to individual cut selection heuristics, whereas we take SCIP's default selection,
which comprises multiple heuristics, as our baseline.

In \cite{xavier2020mluc}, the authors use machine learning techniques to improve MIP solver performance by predicting affine subspaces where the optimal solution is likely to lie. This is similar to cut 
selection in the sense that the space of solutions considered is restricted to obtain faster solve performance.
However, the fundamental difference to our work is that we do not predict additional constraints, but instead select
from the cuts generated by SCIP. The implication is that our cuts are, by construction, guaranteed not to cut off
an optimal solution, whereas in their work there is a non-zero probability that the added constraints render solutions
that would have been optimal in the original problem infeasible.







==> supercuts_results.tex <==














